Optimal Goal-Reaching Reinforcement Learning via Quasimetric Learning

In goal-reaching reinforcement learning (RL), the optimal value function has a particular geometry, called quasimetric structure. This paper introduces Quasimetric Reinforcement Learning (QRL), a new RL method that utilizes quasimetric models to learn optimal value functions. Distinct from prior approaches, the QRL objective is specifically designed for quasimetrics, and provides strong theoretical recovery guarantees. Empirically, we conduct thorough analyses on a discretized MountainCar environment, identifying properties of QRL and its advantages over alternatives. On offline and online goal-reaching benchmarks, QRL also demonstrates improved sample efficiency and performance, across both state-based and image-based observations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> text/AB_proofs_pre_gen_thm2.tex <==

\section{Proofs}

\begin{proof}[Proof of \Cref{thm:val-qmet-equiv}]
We have shown already $-V^* \in \mqmet(\mathcal{S})$. (See also Proposition~A.4 of \citet{wang2022learning}.)

For any $d \in \mqmet(\mathcal{S})$, define \begin{align*}
    \mathcal{A} & \trieq \mathcal{S} \\
    P(s, s_\mathsf{act}) & \trieq \delta_{s_\mathsf{act}} \tag{$\delta_x$ is the Dirac measure at $x$}\\
    R(s, s') & \trieq -d(s, s').
\end{align*}
Then the optimal value of $(\mathcal{S}, \mathcal{A}, P, R)$  is $-d$, regardless of discounting factor (if any).

\psm{}{
For the on-policy values, consider action space $\mathcal{A} = \{a_\mathsf{self}, a_\mathsf{next}\}$. Assume state-space $\size{\mathcal{S}} > 2$. Let $s_1$, $s_2$, $s_3$ be three distinct states in $\mathcal{S}$, all transitions have reward $-1$, and \begin{align}
    P(s_1, a_\mathsf{self}) & = \delta_{s_1} \notag\\
    P(s_2, a_\mathsf{self}) & = \delta_{s_2} \notag\\
    P(s_3, a_\mathsf{self}) & = \delta_{s_3} \tag{$a_\mathsf{self}$ is always a self-transition}\\
    P(s_1, a_\mathsf{next}) & = \delta_{s_2} \notag\\
    P(s_2, a_\mathsf{next}) & = \delta_{s_3} \notag\\
    P(s_3, a_\mathsf{next}) & = \delta_{s_1} \tag{$a_\mathsf{next}$ goes to the next state cyclically}\\
    \pi(s_1; s_2) & = \delta_{a_\mathsf{next}} \tag{$\pi$ always takes $a_\mathsf{next}$ when tasked to go to $s_2$ from $s_1$} \\
    \pi(s_2; s_3) & = \delta_{a_\mathsf{next}} \notag\\
    \pi(s_1; s_2) & = \delta_{a_\mathsf{self}}. \notag
\end{align}
So \begin{align*}
    -V^\pi(s_1; s_2) = -V^{\pi}(s_2; s_3) & = 1 \\
    -V^\pi(s_3; s_1) & = \infty,
\end{align*}
violating triangle-inequality.
}
\end{proof}



\begin{proof}[Proof of \Cref{thm:qrl-exact-recovery}]
Since the transition dynamics is deterministic, we can say that states $s_0$ is locally connected to state $s_1$  if $\exists a \in \mathcal{A}$ such that $P(s_1 \given s_0, a) = 1$. We say a path $(s^\mathsf{path}_{0}, s^\mathsf{path}_{1}, s^\mathsf{path}_{2}, \dots, s^\mathsf{path}_{T})$ connects $s_0$ to $s_1$ if \begin{align*}
    s^\mathsf{path}_{0} & = s_0 \\
    s^\mathsf{path}_{i} & \text{ is locally connected to } s^\mathsf{path}_{i + 1}, \quad \forall i \in \{0, 1, \dots, T - 1\} \\
    s^\mathsf{path}_{T} & = s_1.
\end{align*}
And we say the total cost of this path is the total rewards over all $T-1$ transitions, \ie, $T - 1$.

From the definition of $V^*$ and \Cref{thm:val-qmet-equiv}, We know that, \begin{align}
    -V^* & \in \mqmet(\mathcal{S}) \notag \\
    -V^*(s; g) & = \textsf{total cost of shortest path connecting $s$ to $g$}, \qquad \forall s, g. \notag
\end{align}

Therefore, the constraints stated in \Cref{eq:qrl-ideal-objective} is feasible. The rest of this proof focuses only on $d_\theta$'s that satisfy the constraints.

Due to triangle inequality, we have $\forall s, g$, \begin{equation}
    d_\theta(s_0, g) \leq \textsf{total cost of shortest path connecting $s$ to $g$}.
\end{equation}

Therefore, \begin{equation}
    \mathbb{E}_{s, g} d_\theta(s, g) \leq \mathbb{E}_{s, g} - V^*(s; g),
\end{equation}
with equality iff $d_\theta(s, g) = -V^*(s; g)$ almost surely.

Hence, $d_\theta(s, g) = -V^*(s; g)$ almost surely.

\end{proof}

We first state the formal version of \Cref{thm:qrl-func-approx}.


\begin{theorem}[Function Approximation; Formal]\label{thm:qrl-func-approx-formal}
Assume $\mathcal{S}$ is compact and $V^*$ is continuous. 

Consider a \qmet model that is a universal approximator of $\mqmet(\mathcal{S})$ in terms of $L_\infty$ error. Concretely, $\forall \eps > 0$, we can have $\{d^{(\eps)}_\theta\}_\theta$ such that, there exists some $\theta$ where \begin{equation}
   \forall s_0, s_1 \in \mathcal{S},\quad \abs{d^{(\eps)}_\theta(s_0, s_1) + V(s_0; s_1)} \leq \eps.
\end{equation}


Now consider solving  \Cref{eq:qrl-ideal-objective} over $\{d^{(\eps/2)}_\theta\}_\theta$ with the relaxed constraint, where \begin{equation}
    \forall (s, a, s')~\mathsf{transition},\quad \abs{d^{(\eps/2)}_\theta(s, s') - 1} \leq \eps,
\end{equation}
then for $s \sim p_\mathsf{state}, g \sim p_\mathsf{goal}$,  we have \begin{equation*}
    d_{\theta^*}(s, g) \in [-V^*(s; g) - 1, -(1 + \eps) V^*(s; g)],
\end{equation*}
with probability $1 - o(-\eps\cdot \mathbb{E}[V^*])$.
\end{theorem}

We start by proving a lemma.

\begin{lemma} \label{lemma:relaxed-qrl-lb}
With the assumptions of \Cref{thm:qrl-func-approx-formal}, there exists a $d^{(\eps/2)}_{\theta^\dagger}$ that satisfies the constraint with 
\begin{equation}
    \mathllap{\forall s, g,\quad}
    d^{(\eps/2)}_{\theta^\dagger}(s, g) \geq -\psm{(1 - \frac{\eps}{2})}{(1 + \frac{\eps}{2})}~ V^*(s; g) - \frac{\eps}{2}.
\end{equation}
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:relaxed-qrl-lb}]
\psm{
    Consider any $d^{(\eps/2)}_{\theta'}$ such that \begin{equation}
    \forall (s, a, s')~\mathsf{transition},\quad \abs{d^{(\eps/2)}_\theta(s, s') - 1} \leq \frac{\eps}{2}.
\end{equation}
    By the definition of the universal approximator, $d^{(\eps/2)}_{\theta'}$ exists. 

    For any $(s, g)$, consider any path $(s, s_1, s_2, \dots, s_{T-1}, g)$ connecting $s$ to $g$ (see Proof of \Cref{thm:qrl-exact-recovery} for exact definition). 

    Then, by the definition of $d^{(\eps/2)}_{\theta'}$, we have  \begin{equation}
        (1 + \frac{\eps}{2}) T
        \geq 
        \underbracket{d^{(\eps/2)}_{\theta'}(s; s_1) + \sum_{t=1}^{T-2} d^{(\eps/2)}_{\theta'}(s_t; s_{t+1}) + d^{(\eps/2)}_{\theta'}(s_{T-1}; g)}_{\textsf{total path  cost according to $d^{(\eps/2)}_{\theta'}$} }
        \geq (1 - \frac{\eps}{2}) T \geq -(1 - \frac{\eps}{2}) V^*(s; g). \label{eq:d_eps2_bnd}
    \end{equation}

    Define a new \qmet $d$: \begin{equation}
        \forall s, g, \qquad d(s, g) \trieq \min_{\textsf{path $s \rightarrow g$}} \textsf{total path  cost according to $d^{(\eps/2)}_{\theta'}$}.
    \end{equation}
    
    Then, \Cref{eq:d_eps2_bnd} tells us \begin{equation}
        \forall s, g, \qquad d(s, g) \geq -(1 - \frac{\eps}{2}) V^*(s; g).
    \end{equation}

    % $\forall s, g$, let $\mathsf{path}^*(s \rightarrow g)$ be the true minimum-cost path connecting $s$ to $g$ of length $-V^*(s; g)$. Then, by definition of $d$, we have \begin{equation}
    %     d(s, g) \leq \textsf{total path cost of $\mathsf{path}^*(s \rightarrow g)$ according to $d^{(\eps/2)}_{\theta'}$}.
    % \end{equation}
    % Invoking \Cref{eq:d_eps2_bnd} again tells us \begin{equation}
    %     d(s, g) \leq \textsf{total path cost of $\mathsf{path}^*(s \rightarrow g)$ according to $d^{(\eps/2)}_{\theta'}$} \leq -(1 + \frac{\eps}{2}) V(s; g).
    % \end{equation}

    By universal approximation,  there exists $d^{(\eps/2)}_{\theta^\dagger}$ such that \begin{equation}
        \forall s, g,\quad \abs{ d^{(\eps/2)}_{\theta^\dagger}(s, g) - d(s, g) } \leq \frac{\eps}{2}.
    \end{equation}

    Then, \begin{equation}
        \forall s, g,\quad d^{(\eps/2)}_{\theta^\dagger}(s, g)
        \geq d(s, g) - \frac{\eps}{2} 
        \geq -(1 - \frac{\eps}{2}) V^*(s; g) - \frac{\eps}{2}.
    \end{equation}
}{%
{
$-(1 + \frac{\eps}{2}) V^*$ is a \qmet on $\mathcal{S}$. By universal approximation, there exists $d^{(\eps/2)}_{\theta^\dagger}$  such that \begin{equation}
        \forall s, g,\quad \abs{ d^{(\eps/2)}_{\theta^\dagger}(s, g) + (1 + \frac{\eps}{2}) V^* } \leq \frac{\eps}{2}.
    \end{equation}
    Then, \begin{equation}
        \forall s, g,\quad d^{(\eps/2)}_{\theta^\dagger}(s, g)
        \geq -(1 + \frac{\eps}{2}) V^*(s; g) - \frac{\eps}{2} 
        \geq -(1 + \frac{\eps}{2}) V^*(s; g) - \frac{\eps}{2}.
    \end{equation}
}}
\end{proof}

Now we are ready to prove the \Cref{thm:qrl-func-approx,thm:qrl-func-approx-formal}.


\begin{proof}[Proof of \Cref{thm:qrl-func-approx,thm:qrl-func-approx-formal}]

Let $d^{(\eps/2)}_{\theta^*}$ be the solution to the relaxed problem. By the definition of the universal approximator, such solutions exist.  Moreover, we have \begin{equation}
    \forall s, g, \quad d^{(\eps/2)}_{\theta^*}(s, g) \leq -(1 + \eps) V^*(s; g),\label{eq:sol-ubd}
\end{equation}
by the constraint and triangle inequality.

Define \begin{equation}
    p \trieq \mathbb{P}[ d^{(\eps/2)}_{\theta^*}(s, g) < -V^*(s;g) - 1 ].\label{eq:sol-p-lbd}
\end{equation}

Then \begin{equation}
    \mathbb{E}[d^{(\eps/2)}_{\theta^*}(s, g)] \leq -(1+\eps)\mathbb{E}[V^*(s; g)] - p ,\label{eq:ineq1}
\end{equation} 
where we used \Cref{eq:sol-ubd,eq:sol-p-lbd}.


Let $d^{(\eps/2)}_{\theta^\dagger}$ be the \qmet from \Cref{lemma:relaxed-qrl-lb}. Then, by optimality, we must have \begin{equation}
    \mathbb{E}[d^{(\eps/2)}_{\theta^*}(s, g)] \geq  \mathbb{E}[d^{(\eps/2)}_{\theta^\dagger}(s, g)] \geq -\psm{(1 - \frac{\eps}{2})}{(1 + \frac{\eps}{2})} \mathbb{E}[V^*(s; g)] - \frac{\eps}{2}.\label{eq:ineq2}
\end{equation}


Combining \Cref{eq:ineq1,eq:ineq2}, we have \begin{equation}
    -(1+\eps)\mathbb{E}[V^*(s; g)] - p \geq -\psm{(1 - \frac{\eps}{2})}{(1 + \frac{\eps}{2})} \mathbb{E}[V^*(s; g)] - \frac{\eps}{2}.
\end{equation}

Rearranging the terms, we have \begin{align}
    p 
    & \leq \psm{(1 - \frac{\eps}{2})}{(1 + \frac{\eps}{2})} \mathbb{E}[V^*(s; g)] + \frac{\eps}{2} -(1+\eps)\mathbb{E}[V^*(s; g)]\\
    & \leq - \psm{\frac{3\eps}{2}}{\frac{\eps}{2}} \mathbb{E}[V^*(s; g)] + \frac{\eps}{2}\\
    & \in o(-\eps\ \mathbb{E}[V^*(s; g)] ), \label{eq:qrl-approx-final-lbd}
\end{align}

Combining \Cref{eq:qrl-approx-final-lbd,eq:sol-ubd} gives the desired result.
\end{proof}

==> text/OUTLINE_A.tex <==

%\section{Introduction}
% \input{text/01_introduction}

% \input{text/02_real_world_information}

% \input{text/03_denoise}

% \input{text/04_related}

\section{Introduction}

One approach to modeling decision making problems is via dynamic programming, where the fundamental data structure is the the cost-to-go function, aka the value function. Such a function allows boostrapping, where a complicated decision is broken up into a series of subproblems. Once a subproblem is solved, its subgraph can be collapsed into a single node whose cost is summarized by the value function. This approach is very popular and shows up in nearly all contemporary RL and planning algorithms. 

In deep Rl, value functions are modeled with general neural nets. Most RL algorithms focus on optimizing toward a single goal. In this setting, the value function V(s) reports the cost-to-go to achieve that single goal. In this setting V can be any function V: s --> R, that is, for any V:s --> R, there exists an MDP for which that V is the optimal value func tion. This justifies using very flexible neural net models of V.

However, additional structure emerges when we switch instead to the multi-task setting, where the value function models the cost-to-go to a set of goals. Here, we model V(s,g). In this setting, the true optimal value function, for any MDP, is always a quasimetric function~\cite{XX}. This fact has not been exploited by previous RL algorithms (except a bit in recent work X, Y, Z). One reason for the oversight may be that relatively little work has targeted the multi-task setting.

Given this structure, it's natural to constrain value function search to the space of quasimetrics. This way we are searching for the true value function in a space that is much smaller than the space of all functions s-->R, and we are guaranteed that the true value function lies in this subspace.

This motivates us to design a fundamentally new RL algorithm built around learning quasimetric value functions. A first idea might be to simply run standard RL with value functions parameterized as quasimetrics. This can work decently, as we will show in the experiments, but there is opportunity to go further. Using quasimetric structure allows us to rethink the entire RL optimization process and arrive at an alternative approach that is more efficient and enjoys stronger guarantees than standard RL + quasimetric V.

ChatGPT's version:
``Modeling decision-making problems through dynamic programming often involves using the cost-to-go function, also known as the value function. This function allows for breaking down complex decisions into smaller subproblems and collapsing them into a single node with a summarized cost. However, in the multi-task setting, where the value function models the cost-to-go to a set of goals, additional structure emerges. The true optimal value function in this setting is always a quasimetric function. Despite this, previous RL algorithms have not exploited this fact, but our new algorithm aims to change that by constraining the value function search to the space of quasimetrics and redesigning the entire RL optimization process for more efficiency and stronger guarantees."

Super rough: The new optimization algorithm is in the family of geometric approaches to value function learning, which find a global state embedding from local distance estimates. Obtaining local distance estimates is easy because the cost of a single transition is by definition given by the reward function. So the hard part is to globalize. This is a problem studied in many fields such as metric learning (cite lle, isomap, etc), contrastive learning, etc. The basic idea is to find an embedding such that local distances are preserved and otherwise states are spread out. Why spread out? Because we assume that if we don't observe a local relationship than the two states must be nonlocal, i.e. more than some radius apart, or in the RL setting, the assumption is there is no transition between those states and so the min path between them must be at least two transitions (for simplicity, we will assume unitary cost of each transition, but this can be relaxed). One could apply metric learning to value functions and indeed that's what some other people did (Ge's paper, contrastive RL, etc). But that's the wrong thing to do, since in general value functions are not metrics, they are quasimetrics. So we instead show how to apply this strategy with quasimetrics. We find a quasimetric space in which local relationships are preserved but otherwise states are maximally spread out. We already said why spreading out is good. Why maximally? Because, assuming unitary transition costs for simplicity, the embedding that maximizes the separation of states A and B, subject to constraint that local distances are preserved (adjacent states are unit distance apart), is exactly the length of the shortest path from A to B. It can't be longer because that would violate the constraint. It can't be shorter because that would violate the max. Think of it like a chain with several links. If you pull the chain ends apart, then the distance between the ends is exactly equal to the length of all the links.


\todo{write something about our new objective relying on quasimetrics}

% Quasimetrics is the correct way to do RL.

Our contributions in this paper are  \begin{itemize}
    \item Based on the connection between value functions and quasimetrics (\fixme{ref}), we propose a new RL objective that utilizes quasimetric models to learn \emph{optimal} goal-reaching value functions. 
    \item We provide theoretical guarantees as well as thorough empirical analysis on a discretized \mntcar environment, highlighting qualitative differences with many existing methods. \fixme{ref}
    \item We augment the proposed method to (optionally) also learn optimal Q-functions and/or policies.
    \item On offline \maze tasks, our method performs extremely well in both single-goal and multi-goal evaluations, improving $> 37\%$ over the best baseline and $> 46\%$ over the \dFOURrl handcoded reference controller.  \fixme{ref}
    \item Our learned value functions can be directly used in conjunction with trajectory modelling and planning methods, improving their performances. \fixme{ref}
    \item On online goal-reaching settings, our method shows improved sample efficiency and performance in both state-based and imaged-based observations, outperforming baselines including using \qmet Q-function models with existing standard RL algorithms \citep{liu2022metric}.
\end{itemize}

% 1.25p here

\section{Value Functions are Exactly Quasimetrics}

This sections covers the preliminaries on goal-reaching RL settings, value functions, and \qmets. We also present a new result showing an equivalence between the latter two.

\subsection{Goal-Reaching Reinforcement Learning}

% \paragraph{Goal-reaching RL.} 
We focus on the goal-reaching RL tasks in the form of $(\mathcal{S}, \mathcal{A}, P, r)$, where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $P \colon \mathcal{S} \times \mathcal{A} \rightarrow \Delta(\mathcal{S})$ is the transition function, and $r \colon \mathcal{S} \times \mathcal{S} \rightarrow \R_{\leq 0}$ is the reward (cost) function for performing a transition between two states.  We use $\Delta(A)$ to denote the set of distributions over set $A$.

Given a target state $s_\mathsf{goal} \in \mathcal{S}$, a goal-conditioned agent $\pi(a \given s; s_\mathsf{goal})$ is tasked to reach $s_\mathsf{goal}$ as soon as possible from the current state $s$. 

% Formally, until the agent reaches the goal, it receives a constant negative reward of $-1$ for each transition \footnote{This can be relaxed to be any cost function that depends on starting and ending states of a transition. We use a constant here for simplicity.}. The agent $\pi$ aims to maximize the expected total reward given any $s$ and $s_\mathsf{goal}$, which equals the negated number of transitions taken. We call this quantity the (goal-conditioned) value function $V^\pi(s; s_\mathsf{goal})$.

Formally, until the agent reaches the goal, it receives a negative reward (cost) $r(s, s')$ for each transition $(s, s')$. The agent $\pi$ aims to maximize the expected total reward given any $s$ and $s_\mathsf{goal}$, which equals the negated total cost. We call this quantity the (goal-conditioned) value function $V^\pi(s; s_\mathsf{goal})$.

There exists a optimal policy $\pi^*$ that is optimal for any $(s, s_\mathsf{goal})$: \begin{equation}
    V^{\pi^*}(s; s_\mathsf{goal}) = \max_\pi V^\pi(s; s_\mathsf{goal}).
\end{equation}
We thus define the optimal value function $V^* = V^{\pi^*}$.

\subsection{Value-Quasimetric Equivalence}

\paragraph{Triangle Inequality.} As observed in previous works \citep{wang2022learning,wang2022iqe,liu2022metric,pitis2020inductive}, the optimal value follows triangle inequality: \begin{equation}
    \forall s_1, s_2, s_3, \quad V^*(s_1; s_2) + V^*(s_2; s_3) \leq V^*(s_1, s_3). \label{eq:v-tri-ineq}
\end{equation}

Intuitively, $V^*(s_1, s_3)$ is the highest value (return) among all agents from $s_1$ to $s_3$; and $V^*(s_1; s_2) + V^*(s_2; s_3)$ can be thought of as the highest value among all agents from $s_1$ to $s_2$ and then to $s_3$, a more restricted set. Therefore, \Cref{eq:v-tri-ineq} holds, and $-V^*$ is just like a metric function, except that it may be \emph{asymmetrical}. 

\paragraph{Quasimetrics} is a generalization of metrics that it does not require symmetry. For a set $\mathcal{X}$, a \qmet is a function $d \colon \mathcal{X} \times \mathcal{X} \rightarrow \R_{\geq 0}$ such that \begin{align}
    \forall x_1, x_2, x_3,& \quad d(x_1, x_2) + d(x_2, x_3) \geq d(x_1, x_3) \\
    \forall x, & \quad d(x, x) = 0.
\end{align}
We use $\mqmet(\mathcal{X})$ to denote all such quasimetrics over $\mathcal{X}$.

\Cref{eq:v-tri-ineq} shows that $-V^* \in \mqmet(\mathcal{S})$. In fact, we show that, for any $d \in \mqmet(\mathcal{S})$, $-d$ is the optimal value function for some goal-reaching RL task.

\begin{theorem}[Value-Quasimetric Equivalence]\label{thm:val-qmet-equiv}
    \begin{equation}
    \begin{split}
        \mqmet(\mathcal{S}) = \{-V^* \colon V^* &\text{ is the optimal value for} \\
        &\hspace{1em}\text{   some goal-reaching task}\}
    \end{split}
    \end{equation}
\end{theorem}

\todo{move proof to appendix}
\begin{proof}
We have shown already $-V^* \in \mqmet(\mathcal{S})$. (See also Proposition~A.4 of \citet{wang2022learning}.)

For any $d \in \mqmet(\mathcal{S})$, define \begin{align*}
    \mathcal{A} & \trieq \mathcal{S} \\
    P(s, s_\mathsf{act}) & \trieq \delta_{s_\mathsf{act}} \tag{$\delta_x$ is the Dirac measure}\\
    r(s, s') & \trieq -d(s, s').
\end{align*}
Then the optimal value of $(\mathcal{S}, \mathcal{A}, P, r)$  is $-d$, regardless of discounting factor (if any).
\end{proof}

\begin{figure}
    \centering
    \includegraphics[scale=0.21, trim=145 370 680 160, clip]{figures/single_multi_goal.pdf}
    \caption{\fixme{}}
    \label{fig:structure-multi-goal}
\end{figure}

\paragraph{Structure emerges in multi-goal settings.}
Thus, \qmet is the \emph{exact} function class for goal-reaching RL, and has the best inductive bias. In contrast, any specific-goal value function $V^*(\cdot; s_\mathcal{goal})$ can be \emph{arbitrary} function $\mathcal{S} \rightarrow \R$. In other words, going from traditional single-task RL to multi-task RL, we may have a harder problem, but also have much more structures to utilize (\Cref{fig:structure-multi-goal}). 

\paragraph{Quasimetric Models} refer to parametrized models of quasimetrics $d_\theta \in \mqmet(\mathcal{S})$, where $\theta$ is the parameter to be optimized. Recently, many neural-network-based \qmet models are proposed \citep{wang2022learning,wang2022iqe,pitis2020inductive}. Such models are fully \emph{differentiable},  can be optimized \wrt any differentiable objective, and can potentially generalize to unseen inputs (due to neural networks). 

In the following section, we will show a new RL objective for training \emph{optimal} value function that utilizes the above insights (\eg, \Cref{thm:val-qmet-equiv}) and such \qmet models.

\subsection{Equivalence between V-fn and quasimetrics}

Search space. Non-goal conditional?

Set of Quasimetrics  == Set of Optimal V-fn of MDPs 
(also == set of on-policy V-fn of MDPs.)

So we have the exact correct inductive bias!

\subsection{From local to global: Representing long-horizon (range?) values with locally-consistent quasimetrics}

RL is all about propagating local information to global.  This is usually done by either TD or rolling out a learned model over a long time period. 

Model? (High-level) difference from prior works.

Quasimetrics provide an **alternative** way to characterize global information using local ones.

Assume deterministic dynamics.

Let \begin{equation}
    \mathcal{N} \subset (\mathcal{S} \times \mathcal{S}) \trieq \textsf{Valid Transitions},
\end{equation}
%possibly not containing all posible transitions, \eg, due to incomplete dataset or insufficient exploration.

For any starting state $s_\mathsf{start} \in \mathcal{S}$ target $s_\mathsf{goal} \subset \mathcal{S}$, we can write: \begin{equation}
\begin{split}
    & V(s_\mathsf{start}; s_\mathsf{goal}) = -\max_{\substack{d \subset \mathbb{QMET}(\mathcal{S})}} d(s_\mathsf{start}, s_\mathsf{goal}) \\
    & \qquad\qquad \textsf{subject to}~ \forall (s, s') \in \mathcal{N}, d(s, s') = 1
\end{split}
\end{equation}

\begin{theorem}[Exact Recovery]
Since the optimal V is a quasimetric, we can simultaneous maximize over all pairs to obtain the V function \begin{equation}
\begin{split}
    & V = -\max_{\substack{d \subset \mathbb{QMET}(\mathcal{S})}} \mathbb{E}_{s_\mathsf{start}, s_\mathsf{goal}} [d(s_\mathsf{start}, s_\mathsf{goal})] \\
    & \qquad\qquad \textsf{subject to}~ \forall (s, s') \in \mathcal{N}, d(s, s') = 1
\end{split}
\end{equation}
\end{theorem}

\begin{theorem}
If we instead solve the above equation using a quasimetric approximator and relax the exact $=1$ to be within $\epsilon$ (still for all pairs), the guarantees are ....
\end{theorem}

% Quasimetrics that are consistent w/ observed transitions (restricted qmet space): \begin{equation}
%     \mathbb{QMET}_{\mathcal{N}, \epsilon}(\mathcal{S}) \trieq \left\{ d \subset \mathbb{QMET}(\mathcal{S}) \right\}
% \end{equation}

% \begin{equation}
%     V(s; g) = \max_{d \subset \mathbb{QMET}(\mathcal{S})} d(s, g) 
% \end{equation}


\section{Preliminaries on Embedding-Based Quasimetric Models}

Quickly talk about embedding-based qmet models as universal approx. state their approximation guarantees (maybe informally). 

% 2.5 p here

\section{Quasimetric Reinforcement Learning}

Similar to many RL works \citep{janner2022diffuser,janner2021offline,emmons2021rvs,chen2021decision,paster2022you,yang2022dichotomy}, we assume that $T$ is deterministic.

Motivation: inductive bias, new algorithm, no td, solving subproblems (not just X->G, but also X->Y) etc.

Basic algorithm for learning the value function and latent transition

\begin{align}
    d(x, y) 
    & \trieq d_z(\overbracket{f}^{\mathclap{\textsf{encoder}}}(x), f(y)) \\
    & \trieq d_z(z_x, \underbracket{z_y}_{\mathrlap{\textsf{shorthand for $f(y)$}}}).  \\
    V(s; g) 
    & \trieq -d(s, g).
\end{align}

Goal-conditional distance/V-fn objective (intuitive):

\begin{equation}
\begin{split}
    &\max_{d}~\mathbb{E}_{\substack{s\sim p_\mathsf{state}\\g \sim p_\mathsf{goal}}}[ d(s, g) ] \\
    & \quad\quad \text{subject to } \mathbb{E}_{\substack{(s, a, s') \sim p_\mathsf{transition}}}[ (d(s, s') - 1)^2] \leq \underbracket{\epsilon}_{\mathclap{\textsf{a small positive value}}}
\end{split}
\end{equation}

% 3.75 p here

\subsection{Comparison with Other RL Approaches}

Discuss some potential advantages.

Property Table (from slides).

Use discrete mountain car to showcase the fundamental differences (an env where we have GT)

Compare how V-fn evolve during training (vs TD)?

Use greedy 1-step planning for ours.

Show both reward table and visualization of learned value functions.

Ablations are here:
1. Contrastive RL + quasimetric Q  is on-policy w/ quasimetric inductive bias, removing optimality
2. Quasimetric RL + l2 is removing asymmetry

\begin{table}[h]

\label{tab:dismntcar}%
\caption{Discrete Mountain Car.
% \vspace{-20pt}%
}
    \centering
    \resizebox{
      1\linewidth
    }{!}{%
    \renewcommand\normalsize{\small}%
    \normalsize
    \centering
    % \renewcommand{\arraystretch}{1.4}%
    \setlength{\tabcolsep}{5pt}
    \newcommand{\bftab}{\fontseries{b}\selectfont}%
    \renewcommand{\arraystretch}{1.3}%
    % \renewcommand{\arraystretch}{1.2}%
    \begin{tabular}[b]{lccc}
        \toprule
        &  
        &  Original Task
        &  State-Reaching Tasks \\%[-0.5ex]
        \midrule
        \midrule

        \multirow{2}{*}{\vspace{0pt}\shortstack[l]{Quasimetric RL} }
        & Single-Task
        & \fixme{}
        & --- \\

        & Multi-Task
        & \fixme{}
        & \fixme{} \\[0.15cm]

        {\vspace{0pt}Contrastive RL}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\[0.15cm]

        \multirow{2}{*}{\vspace{0pt}MSG}
        & Single-Task
        & \fixme{}
        & --- \\

        & Multi-Task
        & \fixme{}
        & \fixme{} \\[0.15cm]

        {\vspace{0pt}Diffuser}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\
        \midrule

        \multirow{2}{*}{\vspace{0pt}\shortstack[l]{Quasimetric RL Alg.\\+ Symmetric $\ell_2$ Distance} }
        & Single-Task
        & \fixme{}
        & --- \\

        & Multi-Task
        & \fixme{}
        & \fixme{} \\[0.15cm]

        \multirow{2}{*}{\vspace{0pt}\shortstack[l]{Contrastive RL\\ + Quasimetric Q-Function}}
        & \multirow{2}{*}{\shortstack[c]{---}}
        & \multirow{2}{*}{\fixme{}}
        & \multirow{2}{*}{\fixme{}} \\
        
        &
        &
        & \\
        \midrule

        {\vspace{0pt}Oracle (Full Dynamics)}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\

        {\vspace{0pt}Oracle (Dataset Transitions)}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\
        
        \bottomrule
    \end{tabular}%
    }
    \vspace{-2pt}
\end{table}

\subsection{Transition Learning and Q-Function}


Transition objective 

\begin{equation}
\begin{split}
    &\min_{d, T} \mathbb{E}_{\substack{(s, a, s') \sim p_\mathsf{transition}}}[ d_z(T(z_s, a), z_{s'}) + d_z(z_{s'}, T(z_s, a))]
\end{split}
\end{equation}

Talk about how this objective bounds planning error

\begin{equation}
    Q(s, a; g) \trieq -1 - d_z(T(z_s, a), z_g)
\end{equation}


\subsection{Full Algorithm and Policy Learning}


Goal-conditional distance/V-fn objective (implementation)

\begin{equation}
\begin{split}
    &\max_{d}\min_{\alpha > 0}~\mathbb{E}_{\substack{s\sim p_\mathsf{state}\\g \sim p_\mathsf{goal}}}[ \overbracket{\phi}^{\phi \colon\mathrlap{\textsf{a monotonic increasing func.}}}(d(s, g)) ] \\
    & \quad\quad - \alpha \left(\mathbb{E}_{\substack{(s, a, s') \sim p_\mathsf{transition}}}[ (d(s, s') - 1)^2] - \epsilon\right)
\end{split}
\end{equation}

Talk about potential pessimism regularizer, if we do use it.

Policy objective.

Algorithm block

% 5.25 p here

% \subsection{Theoretical Guarantees}

% Assume bounded density on transitions. How well do we recover the GT distances.

% Small transition loss => planning metric error

% 6 p here

% 6.5 p here

\section{Related Work}

% 7 p here

\citep{eysenbach2022contrastive}  ... \citep{ma2022vip} ...
\citep{micheli2020multi} considers using \qmets for multi-task planning, but does not use models that enforces \qmet properties. \citep{liu2022metric} uses \qmet models to parametrize Q-function, and shows improved performance with DDPG \citep{ddpg} and HER \citep{her} on goal-reaching tasks. These prior works mostly only estimate \emph{on-policy} value functions, and relies on iterative policy improvements to train policies.  Our work differs in that we propose a new \qmet-specific RL objective that directly estimates \emph{optimal} value functions.

qlearning bad \citep{lyle2022learning} \citep{fujimoto2022should}

\section{Experiments}

\subsection{Offline Reinforcement Learning}

Maze2d and AntMaze, a more standard task, and also continuous control.

Reward tables. Visualize embeddings and/or policies.

goal-cond maze2d compared methods: \begin{itemize}
    \item quasimetric + MPPI
    \item GT dynamics MPPI
    \item quasimetric + $\pi$
    \item diffuser
    \item diffuser + quasimetric
    \item Contrastive RL
    \item MSG (relabel)
    \item GCBC (relabel)
\end{itemize}

antmaze2d compared methods: \begin{itemize}
    \item quasimetric
    \item Contrastive RL
    \item MSG
    \item GCBC 
\end{itemize}

\subsection{Online Reinforcement Learning}
state-based \texttt{FetchReach}, \texttt{FetchPush}, \texttt{SawyerPush}, \texttt{SawyerBin}.

methods: \begin{itemize}
    \item quasimetric
    \item Contrastive RL
    \item MRN
    \item TD3 + HER
    \item Model-based
    \item GCBC 
\end{itemize}

Maybe multi-task RoboDesk...

Maybe image-based...

% 8.5 p here

\section{Conclusion}

% 9 p here

% \input{text/05_experiments}

% \input{text/06_discussion}


==> text/OUTLINE_B.tex <==

%\section{Introduction}
% \input{text/01_introduction}

% \input{text/02_real_world_information}

% \input{text/03_denoise}

% \input{text/04_related}

\section{Introduction}

Quasimetrics is the correct way to do RL.

We learn \begin{itemize}
\item optimal goal-conditional value function
% \item a latent world model
\end{itemize}

% 1.25p here

\section{Value Functions are Quasimetrics}
Definitions of MDP, quasimetrics, value functions.


General goal-conditional setting. 

\subsection{Equivalence between V-fn and quasimetrics}

Search space. Non-goal conditional?

Set of Quasimetrics  == Set of Optimal V-fn of MDPs 
(also == set of on-policy V-fn of MDPs.)

So we have the exact correct inductive bias!

\subsection{From local to global: Representing long-horizon (range?) values with locally-consistent quasimetrics}

RL is all about propagating local information to global.  This is usually done by either TD or rolling out a learned model over a long time period. 

Model? (High-level) difference from prior works.

Quasimetrics provide an **alternative** way to characterize global information using local ones.

Assume deterministic dynamics.

Let \begin{equation}
    \mathcal{N} \subset (\mathcal{S} \times \mathcal{S}) \trieq \textsf{Valid Transitions},
\end{equation}
%possibly not containing all posible transitions, \eg, due to incomplete dataset or insufficient exploration.

For any starting state $s_\mathsf{start} \in \mathcal{S}$ target $s_\mathsf{goal} \subset \mathcal{S}$, we can write: \begin{equation}
\begin{split}
    & V(s_\mathsf{start}; s_\mathsf{goal}) = -\max_{\substack{d \subset \mathbb{QMET}(\mathcal{S})}} d(s_\mathsf{start}, s_\mathsf{goal}) \\
    & \qquad\qquad \textsf{subject to}~ \forall (s, s') \in \mathcal{N}, d(s, s') = 1
\end{split}
\end{equation}

\begin{theorem}[Exact Recovery]
Since the optimal V is a quasimetric, we can simultaneous maximize over all pairs to obtain the V function \begin{equation}
\begin{split}
    & V = -\max_{\substack{d \subset \mathbb{QMET}(\mathcal{S})}} \mathbb{E}_{s_\mathsf{start}, s_\mathsf{goal}} [d(s_\mathsf{start}, s_\mathsf{goal})] \\
    & \qquad\qquad \textsf{subject to}~ \forall (s, s') \in \mathcal{N}, d(s, s') = 1
\end{split}
\end{equation}
\end{theorem}

\begin{theorem}
If we instead solve the above equation using a quasimetric approximator and relax the exact $=1$ to be within $\epsilon$ (still for all pairs), the guarantees are ....
\end{theorem}

% Quasimetrics that are consistent w/ observed transitions (restricted qmet space): \begin{equation}
%     \mathbb{QMET}_{\mathcal{N}, \epsilon}(\mathcal{S}) \trieq \left\{ d \subset \mathbb{QMET}(\mathcal{S}) \right\}
% \end{equation}

% \begin{equation}
%     V(s; g) = \max_{d \subset \mathbb{QMET}(\mathcal{S})} d(s, g) 
% \end{equation}


\section{Preliminaries on Embedding-Based Quasimetric Models}

Quickly talk about embedding-based qmet models as universal approx. state their approximation guarantees (maybe informally). 

% 2.5 p here

\section{Quasimetric Reinforcement Learning}

Motivation: inductive bias, new algorithm, no td, solving subproblems (not just X->G, but also X->Y) etc.

Basic algorithm for learning the value function and latent transition

\begin{align}
    d(x, y) 
    & \trieq d_z(\overbracket{f}^{\mathclap{\textsf{encoder}}}(x), f(y)) \\
    & \trieq d_z(z_x, \underbracket{z_y}_{\mathrlap{\textsf{shorthand for $f(y)$}}}).  \\
    V(s; g) 
    & \trieq -d(s, g).
\end{align}

Goal-conditional distance/V-fn objective (intuitive):

\begin{equation}
\begin{split}
    &\max_{d}~\mathbb{E}_{\substack{s\sim p_\mathsf{state}\\g \sim p_\mathsf{goal}}}[ d(s, g) ] \\
    & \quad\quad \text{subject to } \mathbb{E}_{\substack{(s, a, s') \sim p_\mathsf{transition}}}[ (d(s, s') - 1)^2] \leq \underbracket{\epsilon}_{\mathclap{\textsf{a small positive value}}}
\end{split}
\end{equation}

% 3.75 p here

\subsection{Comparison with Other RL Approaches}

Discuss some potential advantages.

Property Table (from slides).

Use discrete mountain car to showcase the fundamental differences (an env where we have GT)

Compare how V-fn evolve during training (vs TD)?

Use greedy 1-step planning for ours.

Show both reward table and visualization of learned value functions.

Ablations are here:
1. Contrastive RL + quasimetric Q  is on-policy w/ quasimetric inductive bias, removing optimality
2. Quasimetric RL + l2 is removing asymmetry

\begin{table}[h]

\label{tab:dismntcar}%
\caption{Discrete Mountain Car.
% \vspace{-20pt}%
}
    \centering
    \resizebox{
      1\linewidth
    }{!}{%
    \renewcommand\normalsize{\small}%
    \normalsize
    \centering
    % \renewcommand{\arraystretch}{1.4}%
    \setlength{\tabcolsep}{5pt}
    \newcommand{\bftab}{\fontseries{b}\selectfont}%
    \renewcommand{\arraystretch}{1.3}%
    % \renewcommand{\arraystretch}{1.2}%
    \begin{tabular}[b]{lccc}
        \toprule
        &  
        &  Original Task
        &  State-Reaching Tasks \\%[-0.5ex]
        \midrule
        \midrule

        \multirow{2}{*}{\vspace{0pt}\shortstack[l]{Quasimetric RL} }
        & Single-Task
        & \fixme{}
        & --- \\

        & Multi-Task
        & \fixme{}
        & \fixme{} \\[0.15cm]

        {\vspace{0pt}Contrastive RL}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\[0.15cm]

        \multirow{2}{*}{\vspace{0pt}MSG}
        & Single-Task
        & \fixme{}
        & --- \\

        & Multi-Task
        & \fixme{}
        & \fixme{} \\[0.15cm]

        {\vspace{0pt}Diffuser}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\
        \midrule

        \multirow{2}{*}{\vspace{0pt}\shortstack[l]{Quasimetric RL Alg.\\+ Symmetric $\ell_2$ Distance} }
        & Single-Task
        & \fixme{}
        & --- \\

        & Multi-Task
        & \fixme{}
        & \fixme{} \\[0.15cm]

        \multirow{2}{*}{\vspace{0pt}\shortstack[l]{Contrastive RL\\ + Quasimetric Q-Function}}
        & \multirow{2}{*}{\shortstack[c]{---}}
        & \multirow{2}{*}{\fixme{}}
        & \multirow{2}{*}{\fixme{}} \\
        
        &
        &
        & \\
        \midrule

        {\vspace{0pt}Oracle (Full Dynamics)}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\

        {\vspace{0pt}Oracle (Dataset Transitions)}
        & \shortstack[c]{---}
        & \fixme{}
        & \fixme{} \\
        
        \bottomrule
    \end{tabular}%
    }
    \vspace{-2pt}
\end{table}

\subsection{Transition Learning and Q-Function}


Transition objective 

\begin{equation}
\begin{split}
    &\min_{d, T} \mathbb{E}_{\substack{(s, a, s') \sim p_\mathsf{transition}}}[ d_z(T(z_s, a), z_{s'}) + d_z(z_{s'}, T(z_s, a))]
\end{split}
\end{equation}

Talk about how this objective bounds planning error

\begin{equation}
    Q(s, a; g) \trieq -1 - d_z(T(z_s, a), z_g)
\end{equation}


\subsection{Full Algorithm and Policy Learning}


Goal-conditional distance/V-fn objective (implementation)

\begin{equation}
\begin{split}
    &\max_{d}\min_{\alpha > 0}~\mathbb{E}_{\substack{s\sim p_\mathsf{state}\\g \sim p_\mathsf{goal}}}[ \overbracket{\phi}^{\phi \colon\mathrlap{\textsf{a monotonic increasing func.}}}(d(s, g)) ] \\
    & \quad\quad - \alpha \left(\mathbb{E}_{\substack{(s, a, s') \sim p_\mathsf{transition}}}[ (d(s, s') - 1)^2] - \epsilon\right)
\end{split}
\end{equation}

Talk about potential pessimism regularizer, if we do use it.

Policy objective.

Algorithm block

% 5.25 p here

% \subsection{Theoretical Guarantees}

% Assume bounded density on transitions. How well do we recover the GT distances.

% Small transition loss => planning metric error

% 6 p here

% 6.5 p here

\section{Related Work}

% 7 p here

\section{Experiments}

\subsection{Offline Reinforcement Learning}

Maze2d and AntMaze, a more standard task, and also continuous control.

Reward tables. Visualize embeddings and/or policies.

goal-cond maze2d compared methods: \begin{itemize}
    \item quasimetric + MPPI
    \item GT dynamics MPPI
    \item quasimetric + $\pi$
    \item diffuser
    \item diffuser + quasimetric
    \item Contrastive RL
    \item MSG (relabel)
    \item GCBC (relabel)
\end{itemize}

antmaze2d compared methods: \begin{itemize}
    \item quasimetric
    \item Contrastive RL
    \item MSG
    \item GCBC 
\end{itemize}

\subsection{Online Reinforcement Learning}
state-based \texttt{FetchReach}, \texttt{FetchPush}, \texttt{SawyerPush}, \texttt{SawyerBin}.

methods: \begin{itemize}
    \item quasimetric
    \item Contrastive RL
    \item MRN
    \item TD3 + HER
    \item Model-based
    \item GCBC 
\end{itemize}

Maybe multi-task RoboDesk...

Maybe image-based...

% 8.5 p here

\section{Conclusion}

% 9 p here

% \input{text/05_experiments}

% \input{text/06_discussion}
